ESGSenticNet: A Neurosymbolic Knowledge Base for Corporate Sustainability Analysis

Evaluating corporate sustainability performance is essential to drive sustainable business practices, amid the need for a more sustainable economy. However, this is hindered by the complexity and volume of corporate sustainability data (i.e. sustainability disclosures), not least by the effectiveness of the NLP tools used to analyse them. To this end, we identify three primary challenges - immateriality, complexity, and subjectivity, that exacerbate the difficulty of extracting insights from sustainability disclosures. To address these issues, we introduce ESGSenticNet, a publicly available knowledge base for sustainability analysis. ESGSenticNet is constructed from a neurosymbolic framework that integrates specialised concept parsing, GPT-4o inference, and semi-supervised label propagation, together with a hierarchical taxonomy. This approach culminates in a structured knowledge base of 44k knowledge triplets - ('halve carbon emission', supports, 'emissions control'), for effective sustainability analysis. Experiments indicate that ESGSenticNet, when deployed as a lexical method, more effectively captures relevant and actionable sustainability information from sustainability disclosures compared to state of the art baselines. Besides capturing a high number of unique ESG topic terms, ESGSenticNet outperforms baselines on the ESG relatedness and ESG action orientation of these terms by 26% and 31% respectively. These metrics describe the extent to which topic terms are related to ESG, and depict an action toward ESG. Moreover, when deployed as a lexical method, ESGSenticNet does not require any training, possessing a key advantage in its simplicity for non-technical stakeholders.

==> others <==
Additionally, the neurosymbolic framework used to construct ESGSenticNet differs from traditional lexical derivation methods in sustainability by being both scalable and automated. Unlike existing lexicons that rely on manually annotated anchor words—a costly and time-intensive process—our framework leverages concept parsing and GPT-4o, automating lexicon derivation through neurosymbolic AI. By eliminating the need for extensive manual annotation, this approach effectively enables a significantly larger and more comprehensive extraction of sustainability lexicons, or in our case, concepts.



ABSTRACT

Sustainability topic analysis is a key method for assessing a company's sustainability performance. This task typically involves identifying key themes within the company's sustainability reports, often leveraging NLP methods. However, existing NLP approaches struggle with three distinct challenges—\textit{irrelevance}, \textit{immateriality}, and \textit{limited organisation}. To elaborate, \textit{irrelevance} refers to extracted topics being unrelated to sustainability, \textit{immateriality} describes topic terms as lacking meaningful value for sustainability assessments, and \textit{limited organisation} denotes that extracted topics may not be coherently organised under sustainability frameworks.

To address these challenges, we introduce ESGSenticNet, a publicly available knowledge base for sustainability topic analysis, built from 1,679 SGX sustainability reports. To construct ESGSenticNet, we develop a neurosymbolic framework that primarily combines specialised concept parsing to extract potential concepts, with GPT-4o labelling these extracted concepts according to a hierarchical taxonomy. This labelling is enhanced by a graph-based semi-supervised method that enables the sharing of labels amongst concepts to maximise annotation coverage while limiting costs. The result is 44,232 triples comprising 23,245 unique concepts, with the triples formatted as (concept, relation, sustainability topic)—i.e. (``halve carbon emission'', supports, ``emissions control''). ESGSenticNet can be deployed as a lexical method for topic analysis. In this approach, concepts serve as topic terms that can be matched within a sustainability report, thereby indicating the presence of sustainability topics. The identified topic is determined by the relation in the concept’s associated triple.

We evaluate ESGSenticNet's effectiveness for sustainability topic analysis on 319 sustainability reports from 75 SGX companies (2015–2023), against state-of-the-art NLP topic models and popular sustainability dictionaries. The results show that ESGSenticNet outperforms baselines, achieving 76\% ESG-relatedness  (+26\% improvement) and 84\% ESG action-orientation (+34\% improvement), while capturing a high number of unique ESG terms (359). Here, ESG-relatedness refer to the proportion of topic terms relevant to sustainability, while ESG action-orientation denote the proportion of terms that express actions taken toward ESG. Additionally, a separate human evaluation study on a random sample of 500 concepts shows that ESGSenticNet achieves 86\%+ accuracy in correctly categorising concepts under their respective sustainability topics. While not exhaustive, these results suggest a strong degree of reliability in aligning topic terms with their intended topics during topic analysis. Finally, unlike computationally intensive NLP models, ESGSenticNet requires no training or tuning for sustainability topic analysis, making it an accessible tool for stakeholders regardless of their resources or expertise.



% description of the rules:


To form the knowledge triples, concepts within our knowledge base are labelled according to their relations (Table \ref{tab:relation_descriptions}) with the topics in our taxonomy (Table \ref{tab:taxonomy}). The relations, \textit{`supports'} and \textit{`undermines'}, clarify how concepts advance or impede crucial aspects of corporate sustainability. In contrast, the relation \textit{`aligns with'} does not consider a concept's impact, highlighting a concept's general connection with broader pillars of environmental, social or governance. Additionally, topics are divided according to their different topic types--\textit{pillar, broad, cross-broad, sub, cross-sub}, as shown in Table \ref{tab:category_type_descriptions}, with relations assigned according to rules (section \ref{sec:rules}).
